Localization via Multiple Reconfigurable Intelligent Surfaces Equipped with Single Receive RF Chains

The extra degrees of freedom resulting from the consideration of Reconfigurable Intelligent Surfaces (RISs) for smart signal propagation can be exploited for high accuracy localization and tracking. In this paper, capitalizing on a recent RIS hardware architecture incorporating a single receive Radio Frequency (RF) chain for measurement collection, we present a user localization method with multiple RISs. The proposed method includes an initial step for direction estimation at each RIS, followed by maximum likelihood position estimation, which is initialized with a least squares line intersection technique. Our numerical results showcase the accuracy of the proposed localization, verifying our theoretical estimation analysis.

==> On Arxiv/fig3_revised.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.63500,0.07800,0.18400}%
\definecolor{mycolor2}{rgb}{0.00000,0.44700,0.74100}%
%
\begin{tikzpicture}[scale=1\columnwidth/10cm]

\begin{axis}[%
width=8cm,
height=5cm,
at={(1.011in,0.642in)},
scale only axis,
xmin=-15,
xmax=15,
xlabel style={font=\color{white!15!black}},
xlabel={Transmit Power [dBm]},
ymode=log,
ymin=0.02,
ymax=6.652,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={Positioning RMSE [m]},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
yminorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black},
legend columns=2,
legend pos=north east
]
\addplot [color=mycolor1, line width=1.0pt]
  table[row sep=crcr]{%
-15	0.458550273073984\\
-10	0.257861768226820\\
-5	0.145006328460596\\
0	0.0815430509075197\\
5	0.0458550273073983\\
10	0.0257861768226821\\
15	0.0145006328460598\\
};
\addlegendentry{\small{PEB, 4 RISs}}

\addplot [color=mycolor2, line width=1.0pt, dashed]
  table[row sep=crcr]{%
-15	0.706582337931950\\
-10	0.397340448268749\\
-5	0.223440954231175\\
0	0.125650082304156\\
5	0.0706582337931950\\
10	0.0397340448268748\\
15	0.0223440954231175\\
};
\addlegendentry{\small{PEB, 3 RISs}}

\addplot [color=mycolor1, mark=o, line width=1.0pt, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
-15	5.35476977775404\\
-10	2.49177220647986\\
-5	0.161278996251825\\
0	0.0899918137340033\\
5	0.0691371995170080\\
10	0.0546943676512246\\
15	0.0492382968278465\\
};
\addlegendentry{\small{ML, 4 RISs, FF}}

\addplot [color=mycolor2, mark=o, line width=1.0pt, mark options={solid, mycolor2}, dashed]
  table[row sep=crcr]{%
-15	6.45396874811166\\
-10	3.34883443895480\\
-5	0.232920366618123\\
0	0.120927051591549\\
5	0.0687626214701920\\
10	0.0406078702284715\\
15	0.0246348498552220\\
};
\addlegendentry{\small{ML, 3 RISs, FF}}

\addplot [color=mycolor1, mark=square, line width=1.0pt, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
-15	3.57998629901968\\
-10	1.68862324088331\\
-5	0.319052260058739\\
0	0.131978881321292\\
5	0.0932485709615470\\
10	0.0725237711316077\\
15	0.0708697357435194\\
};
\addlegendentry{\small{ML, 4 RISs, NF}}




\addplot [color=mycolor2, mark=square, line width=1.0pt, mark options={solid, mycolor2}, dashed]
  table[row sep=crcr]{%
-15	6.65200688512510\\
-10	3.43469899092000\\
-5	0.236562388179611\\
0	0.147271673914487\\
5	0.118194626290541\\
10	0.0918055378796242\\
15	0.0875944633506508\\
};
\addlegendentry{\small{ML, 3 RISs, NF}}

\end{axis}

\end{tikzpicture}%

==> On Arxiv/figure_2_camera_ready.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\begin{tikzpicture}[scale=1\columnwidth/10cm]

\begin{axis}[%
width=8cm,
height=5cm,
at={(1.011in,0.642in)},
scale only axis,
xmin=25,
xmax=100,
xtick={ 25,  36,  49,  64,  81, 100},
xlabel style={font=\color{white!15!black}},
xlabel={Number of RIS Unit Elements $L$},
ymode=log,
ymin=0.0788746368099967,
ymax = 1,
%ymax=0.521127751153846,
ytick={0.1, 1},
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={Positioning RMSE [m]},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
yminorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black},
legend columns=2
]
\addplot [color=mycolor1, mark=o, mark options={solid, mycolor1},line width=1.0pt]
  table[row sep=crcr]{%
25	0.174293125100705\\
36	0.139580580195288\\
49	0.116135509147891\\
64	0.0928308402184045\\
81	0.0909059213941892\\
100	0.0837108406944358\\
};
\addlegendentry{DFT}

\addplot [color=mycolor2, mark=o, mark options={solid, mycolor2},line width=1.0pt, dashed]
  table[row sep=crcr]{%
25	0.20784339702774\\
36	0.180304438207342\\
49	0.13209657640226\\
64	0.11098710350464\\
81	0.0854201853545224\\
100	0.0788746368099967\\
};
\addlegendentry{Directive}

\addplot [color=mycolor1, mark=square, mark options={solid, mycolor1},line width=1.0pt]
  table[row sep=crcr]{%
25	0.521127751153846\\
36	0.259184295888563\\
49	0.183496552222617\\
64	0.208741627926607\\
81	0.106536635737883\\
100	0.100345882306094\\
};
\addlegendentry{DFT, $b=2$}

\addplot [color=mycolor2, mark=square, mark options={solid, mycolor2},line width=1.0pt, dashed]
  table[row sep=crcr]{%
25	0.501008372503908\\
36	0.334405521745377\\
49	0.258734285483262\\
64	0.221877934931354\\
81	0.109884415790844\\
100	0.0982707788761033\\
};
\addlegendentry{Directive, $b=2$}

\addplot [color=mycolor1, mark=triangle, mark options={solid, mycolor1},line width=1.0pt]
  table[row sep=crcr]{%
25	0.208339331383997\\
36	0.146989452960623\\
49	0.133324342824423\\
64	0.0982572404892799\\
81	0.127841515701769\\
100	0.0792885750062671\\
};
\addlegendentry{DFT, $b=3$}


\addplot [color=mycolor2, mark=triangle, mark options={solid, mycolor2},line width=1.0pt, dashed]
  table[row sep=crcr]{%
25	0.234273620166086\\
36	0.210618438108436\\
49	0.179012789530954\\
64	0.110504840590779\\
81	0.125521503579091\\
100	0.0906638227119801\\
};
\addlegendentry{Directive, $b=3$}

\end{axis}


\end{tikzpicture}%
